Vandermonde Matrices with Nodes in the Unit Disk and the Large Sieve

We derive bounds on the extremal singular values and the condition number of NxK, with N>=K, Vandermonde matrices with nodes in the unit disk. The mathematical techniques we develop to prove our main results are inspired by a link---first established by by Selberg [1] and later extended by Moitra [2]---between the extremal singular values of Vandermonde matrices with nodes on the unit circle and large sieve inequalities. Our main conceptual contribution lies in establishing a connection between the extremal singular values of Vandermonde matrices with nodes in the unit disk and a novel large sieve inequality involving polynomials in z \in C with |z|<=1. Compared to Baz\'an's upper bound on the condition number [3], which, to the best of our knowledge, constitutes the only analytical result---available in the literature---on the condition number of Vandermonde matrices with nodes in the unit disk, our bound not only takes a much simpler form, but is also sharper for certain node configurations. Moreover, the bound we obtain can be evaluated consistently in a numerically stable fashion, whereas the evaluation of Baz\'an's bound requires the solution of a linear system of equations which has the same condition number as the Vandermonde matrix under consideration and can therefore lead to numerical instability in practice. As a byproduct, our result---when particularized to the case of nodes on the unit circle---slightly improves upon the Selberg-Moitra bound.

==> def.tex <==
% !TEX root = ConditioningVandermonde_arxiv.tex

% To define macros
\makeatletter
\def\iffirsttoken#1#2{
	\expandafter\def\expandafter\@first@token\expandafter{\@car#1\@nil}
	\expandafter\ifx\@first@token#2\relax
	\expandafter\@firstoftwo
 \else
  	\expandafter\@secondoftwo
 \fi
}

% Theorems
\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}   % Turned off theorem numbering
\newtheorem{prop}{Proposition}
\newtheorem{defn}{Definition}
\newtheorem{ex}{Example}
\newtheorem{lem}[thm]{Lemma}

% Triangleq
\renewcommand{\triangleq}{\vcentcolon=}
\newcommand{\reversetriangleq}{=\vcentcolon}

% Sets
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\torus}{\mathbb{T}}

% Inequalities
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}

% Functions
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\abs}[1]{\left| #1 \right|}
\DeclareMathOperator{\sh}{sinh}
\DeclareMathOperator{\ch}{cosh}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\rk}{rank}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\colsp}{colsp}
\DeclareMathOperator{\rowsp}{rowsp}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\vectorize}{vec}

% Real and imaginary parts
\newcommand{\real}{\mathrm{Re}\!}
\newcommand{\imag}{\mathrm{Im}\!}
\renewcommand{\Re}[1]{\real\left\{#1\right\}}
\renewcommand{\Im}[1]{\imag\left\{#1\right\}}

% Notation
%\newcommand{\vandermonde}[2]{\boldsymbol{\mathscr{V}}_{\!\!#1}(#2)}
\newcommand{\vandermonde}[2]{\mathbf{V}_{\!#1}}
\newcommand{\vandermondeMat}[1]{\mathbf{V}_{\!#1}}
\newcommand{\node}{z}
\newcommand{\nbNodes}{K}
\newcommand{\nbSamples}{N}





